Instruction Fusion: Advancing Prompt Evolution through Hybridization

The fine-tuning of Large Language Models (LLMs) specialized in code generation has seen notable advancements through the use of open-domain coding queries. Despite the successes, existing methodologies like Evol-Instruct encounter performance limitations, impeding further enhancements in code generation tasks. This paper examines the constraints of existing prompt evolution techniques and introduces a novel approach, Instruction Fusion (IF). IF innovatively combines two distinct prompts through a hybridization process, thereby enhancing the evolution of training prompts for code LLMs. Our experimental results reveal that the proposed novel method effectively addresses the shortcomings of prior methods, significantly improving the performance of Code LLMs across five code generation benchmarks, namely HumanEval, HumanEval+, MBPP, MBPP+ and MultiPL-E, which underscore the effectiveness of Instruction Fusion in advancing the capabilities of LLMs in code generation.

==> figure/token_count.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{figure/token_count.pdf} % Reduce the figure size so that it is slightly narrower than the column.
\caption{The average token of the instructions and their responses during 10 round of \textit{Evol-Instruct} on 10 random seeds from the seed pool of WizardCoder.}
\label{fig-case-fuse}
\end{figure}

==> table/result_backup.tex <==
\begin{table*}
\caption{Results of experiments on Python benchmarks. The abbreviations 'CL' and 'CLP' denote the base models \textsc{CodeLlama} and \textsc{CodeLlama-Python}, respectively. 'EC' and 'ECP' represent the models fine-tuned with \texttt{evol-codealpaca-v1} and its Python-specific variant. Models and results marked with an asterisk '*' were reproduced by our team. The values in bracket indicate the performance improvement achieved by fine-tuning with instructions generated by IF, as compared to the use of \texttt{evol-codealpaca-v1} alone.}
\small
\centering
\begin{tabular}{l c c c c c c c c}
\toprule
Method &Size &Open-source& HumanEval & HumanEval+ & MBPP & MBPP+  \\\midrule
    GPT4-Turbo&- & -
    &85.4&81.7 &83.0&70.7\\
    GPT3.5-Turbo&-& -
    &72.6&65.9 &81.7&69.4\\
\midrule
    StarCoder&7B& weight\&data
    &24.4&20.7&33.1&28.8\\
    Mistral&7B& weight
    &28.7&23.2&50.1&40.9\\
    \textsc{CodeLlama-Python}&7B & weight
    &37.8&34.1&57.6&45.4\\
    WizardCoder-CLP&7B & weight
    &48.2&40.9&56.6&47.1\\
    Magicoder$\mathcal{S}$-CLP&7B& weight\&data
    &70.7&66.5&68.4&56.6\\
\midrule
    \textsc{CodeLlama-Python}&13B & weight
    &42.7&36.6&61.2&50.9\\
    WizardCoder-CLP&13B & weight
    &64.0&- \\
    StarCoder&15B & weight\&data
    &34.1&29.3&55.1&46.1 \\   
    CodeT5+&16B & weight\&data
    &31.7&26.2&54.6&44.4 \\
    CodeGen-Mono&16B & weight\&data
    &32.9&27.4&52.6&43.6 \\
    \textsc{CodeLlama-Python}-ECP*&13B &-
    &67.7&64.0&66.4&56.4\\
    \textsc{CodeLlama}-ECP*&13B &-
    &66.5&61.6&67.2&57.4\\
    \textsc{CodeLlama}-EC*&13B&-
    &65.2&61.0&68.4&56.1\\
\midrule    
    \textsc{CodeLlama-Python}&34B & weight
    &51.8&42.7&67.2&52.9\\   
    WizardCoder-CLP&34B & weight
    &73.2&64.6 &73.2&59.9\\
    \textsc{CodeLlama-Python}-ECP*&34B &-
    &72.0&65.2&72.2&61.9\\
    \textsc{CodeLlama}-ECP*&34B &-
    &67.7&62.8&70.9&61.2\\  
    \textsc{CodeLlama}-EC*&34B&-
    &67.7&62.2&69.9&60.4\\
\midrule % code llama
    IF-CLP-ECP&13B& weight\&data
    &73.8 (+6.1)&\textbf{69.5} (+5.5)&\textbf{71.7} (+5.3)&\textbf{61.7} (+5.3)\\
    IF-CL-ECP&13B & weight\&data
    &\textbf{75.6} (+9.1)&68.9 (+7.3) &67.9 (+0.7)&58.6 (+1.2)\\
    IF-CL-EC&13B & weight\&data
    &75.0 (+9.8)&68.9 (+7.9)&70.2 (+1.8)&59.4 (+3.3)\\  
\midrule
    IF-CLP-ECP&34B& weight\&data
    &75.6 (+3.6)&69.5 (+4.3)&\textbf{73.7} (+1.5)&62.7 (+0.8)\\
    IF-CL-ECP&34B & weight\&data
    &\textbf{76.8} (+9.1)&\textbf{70.7} (+7.9)&73.2 (+2.3)&62.9 (+1.7)\\
    IF-CL-EC&34B & weight\&data
    &75.0 (+7.3)&\text{70.1} (+7.9)&\textbf{73.7} (+3.8)&\textbf{63.9} (+3.5)\\
    % \midrule 
    % IF&Deepseek Coder&\CPI
    % &6.7B &xxxx&xxxx
    % &71.7&61.7\\
    
    % IF&Deepseek Coder&\CPI,\HPI
    % &6.7B &xxxx&xxxx
    % &73.7&63.2\\
    % \midrule
    \bottomrule 
\end{tabular}

\label{tab-python}
\vspace{-5mm}
\end{table*}
